NuSTAR Observations of Abell 2163: Constraints on Non-thermal Emission

Since the first non-thermal reports of inverse Compton (IC) emission from the intracluster medium (ICM) of galaxy clusters at hard X-ray energies, we have yet to unambiguously confirm IC emission in observations with newer facilities. RXTE detected IC emission in one of the hottest known clusters, Abell 2163 (A2163), a massive merging cluster with a giant radio halo--the presumed source of relativistic electrons IC scattering CMB photons to X-ray energies. The cluster's redshift (z~0.2) allows its thermal and non-thermal radio emission to fit NuSTARS's FOV, permitting a deep observation capable of confirming or ruling out the RXTE report. The IC flux provides constraints on the average magnetic field strength in a cluster. To determine the global diffuse IC emission in A2163, we fit its global NuSTAR spectrum with four models: single (1T) and two-temperature (2T), 1T+power law component (T+IC), and multi-temperature+power law (9T+IC). Each represent different characterizations of the thermal ICM emission, with power law components added to represent IC emission. We find the 3-30 keV spectrum can be described by purely thermal emission, with a global average temperature of kT = (11.8 $\pm$ 0.2) keV. The IC flux is constrained to $<$ $4.0$ $\times$ $10^{-12}$ $erg$ $s^{-1}$ $cm^{-2}$ using the 1T+IC model and $<$ $1.6$ $\times$ $10^{-12}$ $erg$ $s^{-1}$ $cm^{-2}$ with the more physical 9T+IC model, both to 90% confidence levels. Combining these limits with 1.4 GHz diffuse radio data from the VLA, we find the average magnetic field strength to be $>$ $0.22$$\mu$$G$ and $>$ $0.35$$\mu$$G$, respectively, providing the strongest constraints on these values in A2163 to date.

==> mybibliography.tex <==
@ARTICLE{1993ApJ...407L..49B,
       author = {{Bahcall}, Neta A. and {Cen}, Renyue},
        title = "{The Mass Function of Clusters of Galaxies}",
      journal = {\apjl},
     keywords = {Cosmology, Dark Matter, Galactic Clusters, Galactic Mass, X Ray Astronomy, Hubble Constant, Red Shift, Astrophysics, COSMOLOGY: OBSERVATIONS, COSMOLOGY: DARK MATTER, COSMOLOGY: THEORY, GALAXIES: CLUSTERING, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE},
         year = "1993",
        month = "Apr",
       volume = {407},
        pages = {L49},
          doi = {10.1086/186803},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...407L..49B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019A&A...621A..39E,
       author = {{Ettori}, S. and {Ghirardini}, V. and {Eckert}, D. and
         {Pointecouteau}, E. and {Gastaldello}, F. and {Sereno}, M. and
         {Gaspari}, M. and {Ghizzardi}, S. and {Roncarelli}, M. and
         {Rossetti}, M.},
        title = "{Hydrostatic mass profiles in X-COP galaxy clusters}",
      journal = {\aap},
     keywords = {dark matter, X-rays: galaxies: clusters, galaxies: clusters: intracluster medium, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = jan,
       volume = {621},
          eid = {A39},
        pages = {A39},
          doi = {10.1051/0004-6361/201833323},
archivePrefix = {arXiv},
       eprint = {1805.00035},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...621A..39E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2009astro2010S.305V,
       author = {{Vikhlinin}, A. and {Murray}, S. and {Gilli}, R. and {Tozzi}, P. and
         {Paolillo}, M. and {Brandt}, N. and {Tagliaferri}, G. and {Bautz}, M. and
         {Allen}, S. and {Donahue}, M. and {Evrad}, A. and {Flanagan}, K. and
         {Rosati}, P. and {Borgani}, S. and {Giacconi}, R. and {Weisskopf}, M. and
         {Ptak}, A. and {Alexander}, D. and {Pareschi}, G. and {Forman}, W. and
         {Jones}, C.},
        title = "{X-ray Cluster Cosmology}",
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {astro2010: The Astronomy and Astrophysics Decadal Survey},
         year = "2009",
       volume = {2010},
        month = "Jan",
        pages = {305},
archivePrefix = {arXiv},
       eprint = {0903.5320},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009astro2010S.305V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.457.4515R,
       author = {{Rossetti}, M. and {Gastaldello}, F. and {Ferioli}, G. and
         {Bersanelli}, M. and {De Grandi}, S. and {Eckert}, D. and
         {Ghizzardi}, S. and {Maino}, D. and {Molendi}, S.},
        title = "{Measuring the dynamical state of Planck SZ-selected clusters: X-ray peak - BCG offset}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: clusters: intracluster medium, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2016",
        month = "Apr",
       volume = {457},
       number = {4},
        pages = {4515-4524},
          doi = {10.1093/mnras/stw265},
archivePrefix = {arXiv},
       eprint = {1512.00410},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.4515R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017JKAS...50...93K,
       author = {{Kang}, Hyesung},
        title = "{Shock Acceleration Model with Postshock Turbulence for Giant Radio Relics}",
      journal = {Journal of Korean Astronomical Society},
     keywords = {acceleration of particles, cosmic rays, galaxies: clusters: general, shock waves, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Aug",
       volume = {50},
       number = {4},
        pages = {93-103},
          doi = {10.5303/JKAS.2017.50.4.93},
archivePrefix = {arXiv},
       eprint = {1706.03201},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017JKAS...50...93K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...436L..71M,
       author = {{Markevitch}, Maxim and {Yamashita}, Koujun and {Furuzawa}, Akihiro and
         {Tawara}, Yuzuru},
        title = "{Nonisothermality of the Hottest Cluster Abell 2163}",
      journal = {\apjl},
     keywords = {Galactic Clusters, Gas Temperature, Interstellar Gas, K Lines, Imaging Spectrometers, Iron, Isotherms, Astrophysics, GALAXIES: CLUSTERING, X-RAYS: GALAXIES},
         year = "1994",
        month = "Nov",
       volume = {436},
        pages = {L71},
          doi = {10.1086/187635},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...436L..71M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1958ApJS....3..211A,
       author = {{Abell}, George O.},
        title = "{The Distribution of Rich Clusters of Galaxies.}",
      journal = {\apjs},
         year = 1958,
        month = may,
       volume = {3},
        pages = {211},
          doi = {10.1086/190036},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1958ApJS....3..211A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1996ApJ...456..437M,
       author = {{Markevitch}, M. and {Mushotzky}, R. and {Inoue}, H. and
         {Yamashita}, K. and {Furuzawa}, A. and {Tawara}, Y.},
        title = "{Abell 2163: Temperature, Mass, and Hydrostatic Equilibrium}",
      journal = {\apj},
     keywords = {COSMOLOGY: DARK MATTER, COSMOLOGY: DISTANCE SCALE, GALAXIES: CLUSTERS: INDIVIDUAL NAME: ABELL 2163, X-RAYS: GALAXIES, Astrophysics},
         year = "1996",
        month = "Jan",
       volume = {456},
        pages = {437},
          doi = {10.1086/176668},
archivePrefix = {arXiv},
       eprint = {astro-ph/9506090},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...456..437M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...481..593M,
       author = {{Maurogordato}, S. and {Cappi}, A. and {Ferrari}, C. and {Benoist}, C. and
         {Mars}, G. and {Soucail}, G. and {Arnaud}, M. and {Pratt}, G.~W. and
         {Bourdin}, H. and {Sauvageot}, J. -L.},
        title = "{A 2163: Merger events in the hottest Abell galaxy cluster. I. Dynamical analysis from optical data}",
      journal = {\aap},
     keywords = {galaxies: clusters: general, galaxies: kinematics and dynamics, galaxies clusters: individual: A 2163, Astrophysics},
         year = "2008",
        month = "Apr",
       volume = {481},
       number = {3},
        pages = {593-613},
          doi = {10.1051/0004-6361:20077614},
archivePrefix = {arXiv},
       eprint = {0712.2715},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...481..593M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@TECHREPORT{1992eocm.rept..177A,
       author = {{Arnaud}, M.},
        title = "{A2163: an exceptionally hot cluster of galaxies.}",
      journal = {In ESA, Environment Observation and Climate Modelling Through International Space Projects. Space Sciences with Particular Emphasis on High-Energy Astrophysics p 177-178 (SEE N93-23878 08-88)},
     keywords = {Galactic Clusters, Stellar Spectra, Stellar Temperature, X Ray Spectra, Astronomical Satellites, Cosmic Gases, Cosmology, Data Processing, Japanese Spacecraft, Stellar Mass, Astrophysics},
    booktitle = {Environment Observation and Climate Modelling Through International Space Projects},
         year = "1992",
       editor = {{Guyenne}, T. Duc and {Hunt}, James J.},
        month = "Jul",
        pages = {177-178},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992eocm.rept..177A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...573L..69H,
       author = {{Hansen}, Steen H. and {Pastor}, Sergio and {Semikoz}, Dmitry V.},
        title = "{First Measurement of Cluster Temperature Using the Thermal Sunyaev-Zel'dovich Effect}",
      journal = {\apjl},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Theory, Galaxies: Clusters: General, Methods: Numerical, Scattering, Astrophysics, High Energy Physics - Phenomenology},
         year = "2002",
        month = "Jul",
       volume = {573},
       number = {2},
        pages = {L69-L71},
          doi = {10.1086/342094},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205295},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...573L..69H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...649..673R,
       author = {{Rephaeli}, Yoel and {Gruber}, Duane and {Arieli}, Yinon},
        title = "{Long RXTE Observations of A2163}",
      journal = {\apj},
     keywords = {Galaxies: Clusters: General, Galaxies: Clusters: Individual: Alphanumeric: A2163, Galaxies: Magnetic Fields, Radiation Mechanisms: Nonthermal, Astrophysics},
         year = "2006",
        month = "Oct",
       volume = {649},
       number = {2},
        pages = {673-677},
          doi = {10.1086/506310},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606097},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...649..673R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MNRAS.399.1307M,
       author = {{Million}, E.~T. and {Allen}, S.~W.},
        title = "{Chandra measurements of non-thermal-like X-ray emission from massive, merging, radio halo clusters}",
      journal = {\mnras},
     keywords = {magnetic fields, radiation mechanisms: non-thermal, galaxies: clusters: individual: 1E0657-56, A665, A2163, A2255, A2319, A2744, A2219, A576, A1795, A2204, A478, A2029, intergalactic medium, X-rays: galaxies: clusters, Astrophysics},
         year = "2009",
        month = "Nov",
       volume = {399},
       number = {3},
        pages = {1307-1327},
          doi = {10.1111/j.1365-2966.2009.15359.x},
archivePrefix = {arXiv},
       eprint = {0811.0834},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.399.1307M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...373..106F,
       author = {{Feretti}, L. and {Fusco-Femiano}, R. and {Giovannini}, G. and
         {Govoni}, F.},
        title = "{The giant radio halo in Abell 2163}",
      journal = {\aap},
     keywords = {RADIO CONTINUUM: GENERAL, GALAXIES: CLUSTERS: GENERAL, GALAXIES: CLUSTERS: INDIVIDUAL: A2163, INTERGALACTIC MEDIUM, X-RAYS: GALAXIES: CLUSTERS, Astrophysics},
         year = "2001",
        month = "Jul",
       volume = {373},
        pages = {106-112},
          doi = {10.1051/0004-6361:20010581},
archivePrefix = {arXiv},
       eprint = {astro-ph/0104451},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...373..106F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014A&A...562A..60O,
       author = {{Ota}, N. and {Nagayoshi}, K. and {Pratt}, G.~W. and {Kitayama}, T. and
         {Oshima}, T. and {Reiprich}, T.~H.},
        title = "{Investigating the hard X-ray emission from the hottest Abell cluster A2163 with Suzaku}",
      journal = {\aap},
     keywords = {galaxies: clusters: individual: A2163, galaxies: clusters: intracluster medium, X-rays: galaxies: clusters, cosmology: observations, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Feb",
       volume = {562},
          eid = {A60},
        pages = {A60},
          doi = {10.1051/0004-6361/201322878},
archivePrefix = {arXiv},
       eprint = {1312.4120},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...562A..60O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007PASJ...59S..35T,
       author = {{Takahashi}, Tadayuki and {Abe}, Keiichi and {Endo}, Manabu and
         {Endo}, Yasuhiko and {Ezoe}, Yuuichiro and {Fukazawa}, Yasushi and
         {Hamaya}, Masahito and {Hirakuri}, Shinya and {Hong}, Soojing and
         {Horii}, Michihiro and {Inoue}, Hokuto and {Isobe}, Naoki and
         {Itoh}, Takeshi and {Iyomoto}, Naoko and {Kamae}, Tuneyoshi and
         {Kasama}, Daisuke and {Kataoka}, Jun and {Kato}, Hiroshi and
         {Kawaharada}, Madoka and {Kawano}, Naomi and {Kawashima}, Kengo and
         {Kawasoe}, Satoshi and {Kishishita}, Tetsuichi and {Kitaguchi}, Takao and
         {Kobayashi}, Yoshihito and {Kokubun}, Motohide and {Kotoku}, Jun'ichi and
         {Kouda}, Manabu and {Kubota}, Aya and {Kuroda}, Yoshikatsu and
         {Madejski}, Greg and {Makishima}, Kazuo and {Masukawa}, Kazunori and
         {Matsumoto}, Yukari and {Mitani}, Takefumi and {Miyawaki}, Ryohei and
         {Mizuno}, Tsunefumi and {Mori}, Kunishiro and {Mori}, Masanori and
         {Murashima}, Mio and {Murakami}, Toshio and {Nakazawa}, Kazuhiro and
         {Niko}, Hisako and {Nomachi}, Masaharu and {Okada}, Yuu and
         {Ohno}, Masanori and {Oonuki}, Kousuke and {Ota}, Naomi and
         {Ozawa}, Hideki and {Sato}, Goro and {Shinoda}, Shingo and
         {Sugiho}, Masahiko and {Suzuki}, Masaya and {Taguchi}, Koji and
         {Takahashi}, Hiromitsu and {Takahashi}, Isao and {Takeda}, Shin'ichiro and
         {Tamura}, Ken-Ichi and {Tamura}, Takayuki and {Tanaka}, Takaaki and
         {Tanihata}, Chiharu and {Tashiro}, Makoto and {Terada}, Yukikatsu and
         {Tominaga}, Shin'ya and {Uchiyama}, Yasunobu and {Watanabe}, Shin and
         {Yamaoka}, Kazutaka and {Yanagida}, Takayuki and {Yonetoku}, Daisuke},
        title = "{Hard X-Ray Detector (HXD) on Board Suzaku}",
      journal = {\pasj},
     keywords = {instrumentation: detectors, X-rays: general, Astrophysics},
         year = "2007",
        month = "Jan",
       volume = {59},
        pages = {35-51},
          doi = {10.1093/pasj/59.sp1.S35},
archivePrefix = {arXiv},
       eprint = {astro-ph/0611232},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASJ...59S..35T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007PASJ...59S...1M,
       author = {{Mitsuda}, Kazuhisa and {Bautz}, Mark and {Inoue}, Hajime and
         {Kelley}, Richard L. and {Koyama}, Katsuji and {Kunieda}, Hideyo and
         {Makishima}, Kazuo and {Ogawara}, Yoshiaki and {Petre}, Robert and
         {Takahashi}, Tadayuki and {Tsunemi}, Hiroshi and {White}, Nicholas E. and
         {Anabuki}, Naohisa and {Angelini}, Lorella and {Arnaud}, Keith and
         {Awaki}, Hisamitsu and {Bamba}, Aya and {Boyce}, Kevin and
         {Brown}, Gregory V. and {Chan}, Kai-Wing and {Cottam}, Jean and
         {Dotani}, Tadayasu and {Doty}, John and {Ebisawa}, Ken and
         {Ezoe}, Yuichiro and {Fabian}, Andrew C. and {Figueroa}, Enectali and
         {Fujimoto}, Ryuichi and {Fukazawa}, Yasushi and {Furusho}, Tae and
         {Furuzawa}, Akihiro and {Gendreau}, Keith and {Griffiths}, Richard E. and
         {Haba}, Yoshito and {Hamaguchi}, Kenji and {Harrus}, Ilana and
         {Hasinger}, G{\"u}nther and {Hatsukade}, Isamu and
         {Hayashida}, Kiyoshi and {Henry}, Patrick J. and {Hiraga}, Junko S. and
         {Holt}, Stephen S. and {Hornschemeier}, Ann and {Hughes}, John P. and
         {Hwang}, Una and {Ishida}, Manabu and {Ishisaki}, Yoshitaka and
         {Isobe}, Naoki and {Itoh}, Masayuki and {Iyomoto}, Naoko and
         {Kahn}, Steven M. and {Kamae}, Tuneyoshi and {Katagiri}, Hideaki and
         {Kataoka}, Jun and {Katayama}, Haruyoshi and {Kawai}, Nobuyuki and
         {Kilbourne}, Caroline and {Kinugasa}, Kenzo and {Kissel}, Steve and
         {Kitamoto}, Shunji and {Kohama}, Mitsuhiro and {Kohmura}, Takayoshi and
         {Kokubun}, Motohide and {Kotani}, Taro and {Kotoku}, Jun'ichi and
         {Kubota}, Aya and {Madejski}, Greg M. and {Maeda}, Yoshitomo and
         {Makino}, Fumiyoshi and {Markowitz}, Alex and {Matsumoto}, Chiho and
         {Matsumoto}, Hironori and {Matsuoka}, Masaru and {Matsushita}, Kyoko and
         {McCammon}, Dan and {Mihara}, Tatehiko and {Misaki}, Kazutami and
         {Miyata}, Emi and {Mizuno}, Tsunefumi and {Mori}, Koji and
         {Mori}, Hideyuki and {Morii}, Mikio and {Moseley}, Harvey and
         {Mukai}, Koji and {Murakami}, Hiroshi and {Murakami}, Toshio and
         {Mushotzky}, Richard and {Nagase}, Fumiaki and {Namiki}, Masaaki and
         {Negoro}, Hitoshi and {Nakazawa}, Kazuhiro and {Nousek}, John A. and
         {Okajima}, Takashi and {Ogasaka}, Yasushi and {Ohashi}, Takaya and
         {Oshima}, Tai and {Ota}, Naomi and {Ozaki}, Masanobu and
         {Ozawa}, Hideki and {Parmar}, Arvind N. and {Pence}, William D. and
         {Porter}, F. Scott and {Reeves}, James N. and {Ricker}, George R. and
         {Sakurai}, Ikuya and {Sanders}, Wilton T. and {Senda}, Atsushi and
         {Serlemitsos}, Peter and {Shibata}, Ryo and {Soong}, Yang and
         {Smith}, Randall and {Suzuki}, Motoko and {Szymkowiak}, Andrew E. and
         {Takahashi}, Hiromitsu and {Tamagawa}, Toru and {Tamura}, Keisuke and
         {Tamura}, Takayuki and {Tanaka}, Yasuo and {Tashiro}, Makoto and
         {Tawara}, Yuzuru and {Terada}, Yukikatsu and {Terashima}, Yuichi and
         {Tomida}, Hiroshi and {Torii}, Ken'ichi and {Tsuboi}, Yohko and
         {Tsujimoto}, Masahiro and {Tsuru}, Takeshi Go and
         {Turner}, Martin J.~L. . and {Ueda}, Yoshihiro and {Ueno}, Shiro and
         {Ueno}, Masaru and {Uno}, Shin'ichiro and {Urata}, Yuji and
         {Watanabe}, Shin and {Yamamoto}, Norimasa and {Yamaoka}, Kazutaka and
         {Yamasaki}, Noriko Y. and {Yamashita}, Koujun and {Yamauchi}, Makoto and
         {Yamauchi}, Shigeo and {Yaqoob}, Tahir and {Yonetoku}, Daisuke and
         {Yoshida}, Atsumasa},
        title = "{The X-Ray Observatory Suzaku}",
      journal = {\pasj},
         year = "2007",
        month = "Jan",
       volume = {59},
        pages = {S1-S7},
          doi = {10.1093/pasj/59.sp1.S1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASJ...59S...1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ARA&A..40..319C,
       author = {{Carilli}, C.~L. and {Taylor}, G.~B.},
        title = "{Cluster Magnetic Fields}",
      journal = {\araa},
     keywords = {galaxy clusters, intergalactic medium, intracluster medium, cosmic rays, observations: radio, x-ray, Astrophysics},
         year = "2002",
        month = "Jan",
       volume = {40},
        pages = {319-348},
          doi = {10.1146/annurev.astro.40.060401.093852},
archivePrefix = {arXiv},
       eprint = {astro-ph/0110655},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ARA&A..40..319C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018Galax...6..142V,
       author = {{Vacca}, Valentina and {Murgia}, Matteo and {Govoni}, Federica and
         {En{\ss}lin}, Torsten and {Oppermann}, Niels and {Feretti}, Luigina and
         {Giovannini}, Gabriele and {Loi}, Francesca},
        title = "{Magnetic Fields in Galaxy Clusters and in the Large-Scale Structure of the Universe}",
      journal = {Galaxies},
         year = "2018",
        month = "Dec",
       volume = {6},
       number = {4},
        pages = {142},
          doi = {10.3390/galaxies6040142},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018Galax...6..142V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...770..103H,
       author = {{Harrison}, Fiona A. and {Craig}, William W. and {Christensen}, Finn E. and
         {Hailey}, Charles J. and {Zhang}, William W. and {Boggs}, Steven E. and
         {Stern}, Daniel and {Cook}, W. Rick and {Forster}, Karl and
         {Giommi}, Paolo and {Grefenstette}, Brian W. and {Kim}, Yunjin and
         {Kitaguchi}, Takao and {Koglin}, Jason E. and {Madsen}, Kristin K. and
         {Mao}, Peter H. and {Miyasaka}, Hiromasa and {Mori}, Kaya and
         {Perri}, Matteo and {Pivovaroff}, Michael J. and {Puccetti}, Simonetta and
         {Rana}, Vikram R. and {Westergaard}, Niels J. and {Willis}, Jason and
         {Zoglauer}, Andreas and {An}, Hongjun and {Bachetti}, Matteo and
         {Barri{\`e}re}, Nicolas M. and {Bellm}, Eric C. and {Bhalerao}, Varun and
         {Brejnholt}, Nicolai F. and {Fuerst}, Felix and {Liebe}, Carl C. and
         {Markwardt}, Craig B. and {Nynka}, Melania and {Vogel}, Julia K. and
         {Walton}, Dominic J. and {Wik}, Daniel R. and {Alexander}, David M. and
         {Cominsky}, Lynn R. and {Hornschemeier}, Ann E. and {Hornstrup}, Allan and
         {Kaspi}, Victoria M. and {Madejski}, Greg M. and {Matt}, Giorgio and
         {Molendi}, Silvano and {Smith}, David M. and {Tomsick}, John A. and
         {Ajello}, Marco and {Ballantyne}, David R. and {Balokovi{\'c}}, Mislav and
         {Barret}, Didier and {Bauer}, Franz E. and {Blandford}, Roger D. and
         {Brandt}, W. Niel and {Brenneman}, Laura W. and {Chiang}, James and
         {Chakrabarty}, Deepto and {Chenevez}, Jerome and {Comastri}, Andrea and
         {Dufour}, Francois and {Elvis}, Martin and {Fabian}, Andrew C. and
         {Farrah}, Duncan and {Fryer}, Chris L. and {Gotthelf}, Eric V. and
         {Grindlay}, Jonathan E. and {Helfand}, David J. and {Krivonos}, Roman and
         {Meier}, David L. and {Miller}, Jon M. and {Natalucci}, Lorenzo and
         {Ogle}, Patrick and {Ofek}, Eran O. and {Ptak}, Andrew and
         {Reynolds}, Stephen P. and {Rigby}, Jane R. and
         {Tagliaferri}, Gianpiero and {Thorsett}, Stephen E. and
         {Treister}, Ezequiel and {Urry}, C. Megan},
        title = "{The Nuclear Spectroscopic Telescope Array (NuSTAR) High-energy X-Ray Mission}",
      journal = {\apj},
     keywords = {space vehicles: instruments, X-rays: general, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jun,
       volume = {770},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/770/2/103},
archivePrefix = {arXiv},
       eprint = {1301.7307},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...770..103H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%Perri et al. 2017 https://heasarc.gsfc.nasa.gov/docs/nustar/analysis/nustar_swguide.pdf

@ARTICLE{2014ApJ...792...48W,
       author = {{Wik}, Daniel R. and {Hornstrup}, A. and {Molendi}, S. and
         {Madejski}, G. and {Harrison}, F.~A. and {Zoglauer}, A. and
         {Grefenstette}, B.~W. and {Gastaldello}, F. and {Madsen}, K.~K. and
         {Westergaard}, N.~J. and {Ferreira}, D.~D.~M. and {Kitaguchi}, T. and
         {Pedersen}, K. and {Boggs}, S.~E. and {Christensen}, F.~E. and
         {Craig}, W.~W. and {Hailey}, C.~J. and {Stern}, D. and {Zhang}, W.~W.},
        title = "{NuSTAR Observations of the Bullet Cluster: Constraints on Inverse Compton Emission}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, galaxies: clusters: individual: Bullet cluster, intergalactic medium, magnetic fields, radiation mechanisms: non-thermal, X-rays: galaxies: clusters, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Sep",
       volume = {792},
       number = {1},
          eid = {48},
        pages = {48},
          doi = {10.1088/0004-637X/792/1/48},
archivePrefix = {arXiv},
       eprint = {1403.2722},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...792...48W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1987NASCP2464..339B,
       author = {{Boldt}, Elihu A.},
        title = "{The cosmic X-ray background.}",
     keywords = {Astrophysics, Background Radiation, Galactic Nuclei, X Ray Astronomy, X Rays, Albedo, Isotropy, Photons, Power Spectra, Quantum Efficiency, Space Radiation, Active Galactic Nuclei:X-Ray Background, Quasars:X-Ray Background, X-Ray Background:Active Galactic Nuclei, X-Ray Background:Origin, X-Ray Background:Quasars, X-Ray Background:X-Ray Spectra, X-Ray Spectra:X-Ray Background},
    booktitle = {NASA Conference Publication},
         year = "1987",
       volume = {2464},
        month = "Jun",
        pages = {339-378},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987NASCP2464..339B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...670.1010A,
       author = {{Andersson}, K. and {Peterson}, J.~R. and {Madejski}, G.},
        title = "{Application of an XMM-Newton EPIC Monte Carlo Technique to Analysis and Interpretation of Data for the Abell 1689, RX J0658-55, and Centaurus Clusters of Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Clusters: Individual: Name: Abell 1689, galaxies: clusters: individual (1ES 0657-55.8), Galaxies: Clusters: Individual: Name: Centaurus, Methods: Data Analysis, X-Rays: Galaxies: Clusters, Astrophysics},
         year = "2007",
        month = "Dec",
       volume = {670},
       number = {2},
        pages = {1010-1026},
          doi = {10.1086/521915},
archivePrefix = {arXiv},
       eprint = {astro-ph/0612038},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...670.1010A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...440..775K,
       author = {{Kalberla}, P.~M.~W. and {Burton}, W.~B. and {Hartmann}, Dap and
         {Arnal}, E.~M. and {Bajaja}, E. and {Morras}, R. and
         {P{\"o}ppel}, W.~G.~L.},
        title = "{The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI. Final data release of the combined LDS and IAR surveys with improved stray-radiation corrections}",
      journal = {\aap},
     keywords = {surveys, radio lines: ISM, Galaxy: structure, Astrophysics},
         year = 2005,
        month = sep,
       volume = {440},
       number = {2},
        pages = {775-782},
          doi = {10.1051/0004-6361:20041864},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504140},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...440..775K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@MISC{2010xmm..prop..176B,
       author = {{Bourdin}, Herve},
        title = "{Deep observation of A2163: studying a new ``bullet cluster''}",
     keywords = {Groups of Galaxies, Clusters of Galaxies, Supercluster, A2163},
 howpublished = {XMM-Newton Proposal},
         year = "2010",
        month = "Oct",
        pages = {176},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010xmm..prop..176B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011AA...527A..21B,
       author = {{Bourdin}, H. and {Arnaud}, M. and {Mazzotta}, P. and {Pratt}, G.~W. and
         {Sauvageot}, J. -L. and {Martino}, R. and {Maurogordato}, S. and
         {Cappi}, A. and {Ferrari}, C. and {Benoist}, C.},
        title = "{A2163: Merger events in the hottest Abell galaxy cluster. II. Subcluster accretion with galaxy-gas separation}",
      journal = {\aap},
     keywords = {galaxies: clusters: general, intergalactic medium, X-rays: galaxies: clusters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = mar,
       volume = {527},
          eid = {A21},
        pages = {A21},
          doi = {10.1051/0004-6361/201014907},
archivePrefix = {arXiv},
       eprint = {1011.3154},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...527A..21B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2004ApJ...605..695G,
       author = {{Govoni}, F. and {Markevitch}, M. and {Vikhlinin}, A. and
         {van Speybroeck}, L. and {Feretti}, L. and {Giovannini}, G.},
        title = "{Chandra Temperature Maps for Galaxy Clusters with Radio Halos}",
      journal = {\apj},
     keywords = {Galaxies: Clusters: General, Galaxies: Intergalactic Medium, Radio Continuum: Galaxies, X-Rays: Galaxies: Clusters, Astrophysics},
         year = "2004",
        month = "Apr",
       volume = {605},
       number = {2},
        pages = {695-708},
          doi = {10.1086/382674},
archivePrefix = {arXiv},
       eprint = {astro-ph/0401421},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...605..695G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...725.1688A,
       author = {{Ajello}, M. and {Rebusco}, P. and {Cappelluti}, N. and {Reimer}, O. and
         {B{\"o}hringer}, H. and {La Parola}, V. and {Cusumano}, G.},
        title = "{Galaxy Clusters in the Swift/BAT Era. II. 10 More Clusters Detected Above 15 keV}",
      journal = {\apj},
     keywords = {acceleration of particles, galaxies: clusters: general, magnetic fields, radiation mechanisms: non-thermal, X-rays: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2010",
        month = "Dec",
       volume = {725},
       number = {2},
        pages = {1688-1706},
          doi = {10.1088/0004-637X/725/2/1688},
archivePrefix = {arXiv},
       eprint = {1009.4699},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...725.1688A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1994hea..book.....L,
       author = {{Longair}, Malcolm S.},
        title = "{High energy astrophysics. Vol.2: Stars, the galaxy and the interstellar medium}",
         year = "1994",
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994hea..book.....L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1979rpa..book.....R,
       author = {{Rybicki}, George B. and {Lightman}, Alan P.},
        title = "{Radiative processes in astrophysics}",
         year = "1979",
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979rpa..book.....R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...423..111F,
       author = {{Feretti}, L. and {Orr{\`u}}, E. and {Brunetti}, G. and
         {Giovannini}, G. and {Kassim}, N. and {Setti}, G.},
        title = "{Spectral index maps of the radio halos in Abell 665 and Abell 2163}",
      journal = {\aap},
     keywords = {radio continuum: general, galaxies: clusters: general, galaxies: clusters: individual: A665, galaxies: clusters: individual: A2163, galaxies: intergalactic medium, X-rays: galaxies: clusters, Astrophysics},
         year = "2004",
        month = "Aug",
       volume = {423},
        pages = {111-119},
          doi = {10.1051/0004-6361:20040316},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404283},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...423..111F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJS..204...19P,
       author = {{Perley}, R.~A. and {Butler}, B.~J.},
        title = "{An Accurate Flux Density Scale from 1 to 50 GHz}",
      journal = {\apjs},
     keywords = {instrumentation: interferometers, methods: observational, radio continuum: general, techniques: interferometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = feb,
       volume = {204},
       number = {2},
          eid = {19},
        pages = {19},
          doi = {10.1088/0067-0049/204/2/19},
archivePrefix = {arXiv},
       eprint = {1211.1300},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..204...19P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...777..141C,
       author = {{Cassano}, R. and {Ettori}, S. and {Brunetti}, G. and {Giacintucci}, S. and
         {Pratt}, G.~W. and {Venturi}, T. and {Kale}, R. and {Dolag}, K. and
         {Markevitch}, M.},
        title = "{Revisiting Scaling Relations for Giant Radio Halos in Galaxy Clusters}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, radiation mechanisms: non-thermal, radio continuum: general, X-rays: galaxies: clusters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = nov,
       volume = {777},
       number = {2},
          eid = {141},
        pages = {141},
          doi = {10.1088/0004-637X/777/2/141},
archivePrefix = {arXiv},
       eprint = {1306.4379},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...777..141C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.431..394W,
       author = {{Willingale}, R. and {Starling}, R.~L.~C. and {Beardmore}, A.~P. and
         {Tanvir}, N.~R. and {O'Brien}, P.~T.},
        title = "{Calibration of X-ray absorption in our Galaxy}",
      journal = {\mnras},
     keywords = {ISM: abundances, dust, extinction, ISM: molecules, X-rays: ISM, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = may,
       volume = {431},
       number = {1},
        pages = {394-404},
          doi = {10.1093/mnras/stt175},
archivePrefix = {arXiv},
       eprint = {1303.0843},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.431..394W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979ApJ...227..364R,
       author = {{Rephaeli}, Y.},
        title = "{Relativistic electrons in the intracluster space of clusters of galaxies: the hard X-ray spectra and heating of the gas.}",
      journal = {\apj},
     keywords = {Energy Dissipation, Galactic Clusters, Gas Heating, High Energy Electrons, Intergalactic Media, X Ray Spectra, Energy Spectra, Magnetohydrodynamic Waves, Relativistic Particles, Astrophysics, Intergalactic Matter:Heating, Intergalactic Matter:X Rays},
         year = 1979,
        month = jan,
       volume = {227},
        pages = {364-369},
          doi = {10.1086/156740},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...227..364R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999NewA....4..141G,
       author = {{Giovannini}, G. and {Tordi}, M. and {Feretti}, L.},
        title = "{Radio halo and relic candidates from the NRAO VLA Sky Survey}",
      journal = {\na},
     keywords = {Astrophysics},
         year = 1999,
        month = mar,
       volume = {4},
       number = {2},
        pages = {141-155},
          doi = {10.1016/S1384-1076(99)00018-4},
archivePrefix = {arXiv},
       eprint = {astro-ph/9904210},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999NewA....4..141G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...423..111F,
       author = {{Feretti}, L. and {Orr{\`u}}, E. and {Brunetti}, G. and
         {Giovannini}, G. and {Kassim}, N. and {Setti}, G.},
        title = "{Spectral index maps of the radio halos in Abell 665 and Abell 2163}",
      journal = {\aap},
     keywords = {radio continuum: general, galaxies: clusters: general, galaxies: clusters: individual: A665, galaxies: clusters: individual: A2163, galaxies: intergalactic medium, X-rays: galaxies: clusters, Astrophysics},
         year = 2004,
        month = aug,
       volume = {423},
        pages = {111-119},
          doi = {10.1051/0004-6361:20040316},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404283},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...423..111F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


